Rotation Measure study of FRB 20180916B with the uGMRT

Context. Fast Radio Burst 20180916B is a repeating FRB whose activity window has a 16.34 day periodicity that also shifts and varies in duration with the observing frequency. Recently, arxiv:2205.09221 reported the FRB has started to show secular Rotation Measure (RM) increasing trend after only showing stochastic variability around a constant value of $-114.6$ rad m$^{-2}$ since its discovery. Aims. We aim to further study the RM variability of FRB 20180916B. The data comes from the ongoing campaigns of FRB 20180916B using the upgraded Giant Metrewave Radio Telescope (uGMRT). The majority of the observations are in Band 4, which is centered at 650 MHz with 200 MHz bandwidth. Methods. We apply a standard single pulse search pipeline to search for bursts. In total, we detect 116 bursts with $\sim$36 hours of on-source time spanning 1200 days, with two bursts detected during simultaneous frequency coverage observations. We develop and apply a polarization calibration strategy suited for our dataset. On the calibrated bursts, we use QU-fitting to measure RM. Lastly, we also measure various other properties such as rate, linear polarization fraction and fluence distribution. Results. Of the 116 detected bursts, we could calibrate 79 of them. From which, we observed in our early observations the RM continued to follow linear trend as modeled by arxiv:2205.09221. However, our later observations suggest the source switch from the linear trend to stochastic variations around a constant value of $-58.75$ rad m$^{-2}$. We also study cumulative rate against fluence and note that rate at higher fluences (> 1.2 Jy ms) scales as $\gamma = -1.09(7)$ whereas that at lower fluences (between 0.2 and 1.2 Jy ms) only scales as $\gamma = -0.51(1)$, meaning rate at higher fluence regime is steeper than at lower fluence regime.

==> makefile <==
SHELL:=/bin/bash
all:main.tex
	latexmk -pdf -silent 

debug:main.tex
	latex $< ;\
	open main.pdf &

old:main.tex
	latex $< ;\
	bibtex rm ;\
	latex $< ;\
	latex $< ;\
	pdflatex $< ;\
	open main.pdf &

.PHONY: gadd
gadd:
	@read -p "git commit description: " DESCRIPTION;\
	git add . ;\
	git commit -m "$$DESCRIPTION" 

.PHONY: gpush
gpush:
	git push origin;

gpull:
	@read -p "remote name:" REMOTE;\
	git pull $$REMOTE master --allow-unrelated-histories

gcheck:
	git log -p -2

gremote:
	git remote add overleaf $$URLoverleaf
	git remote add github $$URLgithub

.PHONY: clean
clean: 
	rm -f *.dvi  *.aux *.blg *.toc *.out *.fdb_latexmk *.log *.synctex.gz *.fls

